Deep Archetypal Analysis

"Deep Archetypal Analysis" generates latent representations of high-dimensional datasets in terms of fractions of intuitively understandable basic entities called archetypes. The proposed method is an extension of linear "Archetypal Analysis" (AA), an unsupervised method to represent multivariate data points as sparse convex combinations of extremal elements of the dataset. Unlike the original formulation of AA, "Deep AA" can also handle side information and provides the ability for data-driven representation learning which reduces the dependence on expert knowledge. Our method is motivated by studies of evolutionary trade-offs in biology where archetypes are species highly adapted to a single task. Along these lines, we demonstrate that "Deep AA" also lends itself to the supervised exploration of chemical space, marking a distinct starting point for de novo molecular design. In the unsupervised setting we show how "Deep AA" is used on CelebA to identify archetypal faces. These can then be superimposed in order to generate new faces which inherit dominant traits of the archetypes they are based on.

==> 128-paper (2)/a00_deepAT_ABSTRACT_gcpr19.tex <==
\begin{abstract}
Deep Archetypal Analysis (DeepAA) generates latent re\-presentations of high-dimensional datasets in terms of intuitively understandable basic entities called \textit{archetypes}. The proposed method extends linear Archetypal Analysis (AA), an unsupervised method to represent multivariate data points as convex combinations of extremal data points. Unlike the original formulation, Deep AA is generative and capable of handling side information. In addition, our model provides the ability for data-driven representation learning which reduces the dependence on expert knowledge. We empirically demonstrate the applicability of our approach by exploring the chemical space of small organic molecules. In doing so, we employ the archetype constraint to learn two different latent archetype representations for the \textit{same} dataset, with respect to two chemical properties. This type of supervised exploration marks a distinct starting point and let us steer de novo molecular design.




%This type of supervised exploration of chemical space marks a distinct starting point for de novo molecular design.







%Our method is motivated by studies of evolutionary trade-offs in biology where archetypes are species highly adapted to a single task. Along these lines, we %demonstrate that ``Deep AA'' also lends itself to the supervised exploration of chemical space, marking a distinct starting point for de novo molecular %design. In the unsupervised setting we show how ``Deep AA'' is used on CelebA to identify archetypal faces. These can then be superimposed in order to %enerate new faces which inherit dominant traits of the archetypes they are based on.

%used as landmarks for a more intuitive exploration of the whole data






%??????
% feature sclaing domain , combination... and automat ...




%The proposed method is able to (i) learn (ii)

%The proposed method is an extension of linear ``Archetypal Analysis'' (AA) and adresses the following %issues:


%, a method to represent multivariate data points as sparse convex combinations of extremal elements of %the dataset. AA is used e.g. to analyze evolutionary trade-offs in biology.  


%We propose \textit{Deep Archetypal Analysis} an extension of Archetypal Analysis (AA) which is a method %to represent multivariate data points as sparse convex combinations of extremal elements of the dataset.  
\end{abstract}


==> 128-paper (2)/a01_deepAT_INTRO_gcpr19.tex <==
\section{Introduction}
\label{sec_intro}

Archetypal analysis (AA) is of particular interest when a given data set is assumed to be a superposition of various populations or mechanisms. For a given number of $k$ archetypes, linear AA finds an optimal approximation of the data convex hull, i.e. a polytope, with respect to a given loss function. All data points can then be described as convex mixtures of these $k$ extreme points. In evolutionary biology this has led to the interpretation of archetypes as the representatives most adapted to a given task while non-archetypal representatives are described as mixtures of these extreme or pure types -- able to perform a variety of tasks but non of them optimally \cite{shoval2012}. We identified several limitations of the linear AA model which we would like to address. (I) For data points on a linear submanifold, e.g. a plane in $\mathbb{R}^2$, a strictly monotone transformation should in general have no influence on which points are identified as archetypes. But such a transformation would in fact introduce a non-zero curvature to that submanifold. As a consequence it would become impossible for \textit{linear} AA to approximate equally well the data convex hull, given the same number $k$ of archetypes as before. (II) Using linear AA to explore a dataset and uncover meaningful archetypes usually requires some form of prior knowledge. Either by knowing how many archetypes $k$ are necessary to have an acceptable trade-off between interpretability and error \textit{or} by having domain knowledge about which dimensions of the dataset can/should be omitted, scaled or combined. This procedure of injecting \textit{side information} to the exploration of a given dataset is unpractical at best, impossible even if no intuition about a given problem can be formed. Often side information is available in form of scalar labels, but of course side information could be any kind of richly structured data. When learning a representation of the data, linear AA offers no possibility to incorporate such side information by which to guide the selection of an optimal number of archetypes as well as the relevant dimensions. (III) Linear AA is non-generative. But especially the prospect of incorporating differentiated side information makes the ability to generate new samples -- conditioned on that side inormation -- more attractive. Closely related to that is the ability to interpolate which, in the sense of AA, would be expressed as a \textit{geometric} interpolation within a coordinate system spanned by the $k$ archetypes.\\
In the following we will propose solutions to these limitations in order to extend the area of applicability of AA. In short this entails recasting linear AA as a latent space model within the framework of the Deep Variational Information Bottleneck. Of course this means that our extension constitutes a non-linear version of AA. Extentions into non-linearity have been proposed in the past based on kernalization but such frameworks remain less flexible still in comparison to a learned deep network architecture. But with this increase in flexibility comes a certain trade-off: without side information to guide the learning of a meaningful latent representation the result might be without significance as increased flexibility implies a multitude of possible latent representations dependent only on the side information on which any learning process should therefore be conditioned.\\



%The evolutionary development of biological systems is characterized by a fundamental trade-off: If multiple tasks need to be performed, no system can be optimal at all tasks at once. Examples of such trade-offs include those between longevity and fecundity in Drosophila melanogaster where long-lived 
%flies show decreased fecundity \cite{drosophila} or predators that evolve to be fast runners but eventually have to trade-off their ability to subdue large or strong prey, e.g. cheetah versus lion \cite{garland2014}. Such evolutionary trade-offs are known to affect the range of phenotypes found in nature \cite{tendler2015}. In \cite{shoval2012} empirical examples are presented to support the argument that best--trade-off phenotypes are weighted averages of archetypes where archetypes are understood to be phenotypes specialized for a single task. An example of an evolutionary trade-off in the space of traits (or phenospace) for 138 species of bats (Microchiroptera) is shown in Fig. \ref{fig:bats138}. Based on data from \cite{norberg1987} the dominant food habit of each species is represented in a two-dimensional space where the axis depict \textit{Body Mass} and \textit{Wing Aspect Ratio}. The latter is the square of the wingspan divided by the wing area. The indicated archetypes were calculated according to Archetypal Analysis proposed by \cite{cutlerBreiman1994}. Table \ref{tbl_traits} gives an account of the \textit{single} task a given archetype is optimized to perform. 
%
%\begin{figure}[h!]
%\begin{center}
%   \includegraphics[scale=.40]{bats138}
%\end{center}
%\vspace{-1.8em}
%   \caption{Phenospace of 138 species of Microchiroptera. The dominant food habit of each species, and thereby the ability to procure this food source, is linked to the morphology of the animals, e.g. a higher \textit{Wing Aspect Ratio} corresponds with the greater aerodynamic efficiency needed to chase high flying insects. Archetypes are extreme types, optimized to perform a single task. Proximity of a species to an archetype quantifies the level of adaptation this species has undergone with respect to the archetypal task.}
%\label{fig:bats138}
%\end{figure}
%%
%The trade-off situation can be interpreted using Pareto optimality theory \cite{steuer1986} which was recently used in biology to study trade-offs in evolution \cite{schuetz2012,elSamad2005}. All phenotypes that have evolved over time lie within a restricted part of the phenospace, the so-called Pareto front, which is the set of phenotypes that cannot be improved at all tasks simultaneously. If there were a phenotype $p$ being better at all tasks than a second phenotype $p'$ then the latter would be eliminated by natural selection. Consequently phenotypes on the Pareto front are the best possible compromises between the different requirements or tasks.
%
%\begin{table}%[b!]
%\caption{Characteristic traits of the archetypes identified in Fig. \ref{fig:bats138} and the task each archetypal species is optimized to perform.}
%\label{tbl_traits}
%\vskip 0.05in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lccr}
%\toprule
%Archetype & Traits & Task: hunt for...\\
%\midrule
%archetype 1 & \makecell{low aspect ratio,\\ large body} & \makecell{...plant material,\\ nectar \& pollen} \\
%archetype 2 & \makecell{low aspect ratio,\\ small body} & \makecell{...small insects\\ near vegetation} \\
%archetype 3 & \makecell{high aspect ratio,\\ medium body} & \makecell{...high flying,\\ large insects} \\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table}
%
%However, there are several shortcomings associated with Archetypal Analysis: \textit{(i)} Regarding the Microchiroptera example, a total of eight measurements per species were collected by \cite{norberg1987} but selecting the dimensions that would reveal the relation between food habit and phenotype depicted in Fig. \ref{fig:bats138} requires prior knowledge, here in form of knowledge about aerodynamics. \textit{(ii)} A representational problem is introduced when features of different types and from different domains are used. Again referring to Fig. \ref{fig:bats138}, representing the \textit{Body Mass} on a $\log$-scale while the \textit{Wing Aspect Ratio} enters linearly requires expert knowledge or is simply the result of a trial and error process if even a domain expert cannot provide useful insights. \textit{(iii)} Finally, Archetypal Analysis in its original formulation is an \textit{unsupervised} learning process, i.e. side information cannot be taken into account during learning.
%
\subsubsection{Literature} Linear ``Archetypal Analysis'' (AA) was first proposed by Adele Cutler and Leo Breiman \cite{cutlerBreiman1994}. Since its conception AA has known several advancements on the algorithmic as well as the application side. An extension to (non-linear) Kernel AA is proposed by \cite{bauck2014Kernel,morupKernelAA}, algorithmic improvements by adapting a Frank--Wolfe type algorithm to calculate the archetypes are made by \cite{bauck2015FW} and the extension by \cite{seth2016} introduces a probabilistic version of AA. Archetypal style analysis \cite{styleAA} applies AA to the learned image representations in deep neural networks for artistic style manipulation. In \cite{sand2012} the authors are concerned with model selection by asking for the optimal number of archetypes for a given dataset while \cite{kauf2015} addresses in part the shortcoming of AA we describe in the introduction under (ii). Although AA did not prevail as a commodity tool for pattern analysis it has for example been used by \cite{bauck2009ImgCol} to find archetypal images in large image collections or by \cite{can2015} to perform the analogous task for large document collections. For the human genotype data studied by \cite{huggins2007}, inferred archetypes are interpreted as representative populations for the measured genotypes. And in \cite{chan2003} AA is used to analyse galaxy spectra which are viewed as weighted superpositions of the emissions from stellar populations, nebular emissions and nuclear activity.  
% \textit{Note that all contributions cited in this paragraph refer to the original AA model from \cite{cutlerBreiman1994}.}
%
%\textbf{Deep Latent Variable Models} 
%Deep latent variable models have received remarkable attention in recent years %and been applied to a large amount of problems. The most prevalent approaches %are 
%
Our work builds upon Variational Autoencoders (VAEs), arguably the most prevalent representatives of the class of ``Deep Latent Variable Models''. VAEs were introduced by \cite{kingmaWelling2013,rezende2014} and use an inference network to perform a variational approximation of the posterior distribution of the latent variable. Important work in this direction include \cite{KingmaSemi,pmlrrezende15} and \cite{Jang}. More recently, \cite{alemi2016} has discovered a close connection between VAE and the Information Bottleneck principle \cite{tishby2000}. Here, the Deep Variational Information Bottleneck (DVIB) is a VAE where $X$ is replaced by $Y$ in the decoder. Subsequently, the DVIB has been extended in multiple directions such as sparsity \cite{2018arXiv180406216W} or causality \cite{2018arXiv180702326P}.\\
At the same time as our work, \textit{AAnet} was published by \cite{AAnet}. There the authors introduce a neural network based extentension of linear archetypal analysis on the basis of standard non-variational autoencoders. In their work two regularization terms, applied to an intermediate representation provide the latent archetypal convex representation of a non-linear transformation of the input. In contrast to our work which is based on probabilistic generative models (VAE, DVIB), \textit{AAnet} attempts to emulate the generative process by adding noise to the latent representation during training. Further, no side information is incorporated which can -- and in our opinion should -- be used to constrain potentially \textit{over-flexible} neural networks and guide the optimisation process towards learning a meaningful representation. 
%
%Concurrently to our work, we discovered that \cite{AAnet} employ a non-linear AA neural network approach on the basis of (classical) Autoencoders. There, two %regularisation terms applied to an intermediate representation provide the archetypal convex latent representation of a non-linear transformation of the %input data. In contrast to our work, \cite{AAnet} is not based on a probabilistic generative model such as VAE or DVIB but attains the generative capabilites %by imposing noise on the latent representation during training. Further, no side information is incorporated which can constrain the vast flexibility of the %neural network. \colorbox{red}{BATCH PROBLEMATIC?}
%
\subsubsection{Contribution}We propose \textit{Deep Archetypal Analysis} (DeepAA) which is a novel, non--linear extension of the original model proposed by \cite{cutlerBreiman1994}. By introducing \textit{DeepAA} within a DVIB framework we address several issues of the original model. Unlike the original model, \textit{DeepAA} (i) is able to identify meaningful archetypes even on non-linear data manifolds, (ii) does not rely on expert knowledge when combining relevant dimensions or learning appropriate transformations (e.g. scaling) and (iii) is able to incorporate side information into the learning process in order to regularize and guide the learning process towards meaningful latent representations. On a large scale experiment we demonstrate the usefulness of \textit{DeepAA} in a setting with side information on the QM9 dataset which contains the chemical structures and properties of 134 kilo molecules \cite{rudd2012,rama2014}. As modern chemistry and material science are increasingly concerned with material property prediction, we show that \textit{DeepAA} can be used to \textit{systematically} explore vast chemical spaces in order to identify starting points for further chemical optimisation.

%Beside the analysis of evolutionary trade-offs as the motivation for \textit{DeepAA}, we present two large scale experiments: First we show that the %unsupervised exploration of CelebA \cite{celebA2015} using \textit{DeepAA} offers a highly interpretable perspective on the dominant factors of variation as %face images can be characterized as convex mixtures of \textit{archetypal faces}. Second we demonstrate the usefulness of \textit{DeepAA} in a setting with %side information on the QM9 dataset which contains the chemical structures and properties of 134 kilo molecules \cite{rudd2012,rama2014}. As modern chemistry %and material science are increasingly concerned with material property prediction, we show that \textit{DeepAA} can be used to \textit{systematically} %explore vast chemical spaces in order to identify starting points for further chemical optimisation.
%
%\paragraph{Contribution}We propose \textit{Deep Archetypal Analysis} (DeepAA) which is a novel, non--linear extension of the original model proposed by \cite{cutlerBreiman1994}. By introducing \textit{DeepAA} within a VAE framework we address several issues of the original model. Unlike the original model, \textit{DeepAA} (i) does not rely on expert knowledge when combining relevant dimensions, (ii) learns appropriate transformations (e.g. scaling) when combining features of different types and (iii) is able to incorporate side information into the learning process if necessary. Beside the analysis of evolutionary trade-offs as the motivation for \textit{DeepAA}, we present two large scale experiments: First we show that the unsupervised exploration of CelebA \cite{celebA2015} using \textit{DeepAA} offers a highly interpretable perspective on the dominant factors of variation as face images can be characterized as convex mixtures of \textit{archetypal faces}. Second we demonstrate the usefulness of \textit{DeepAA} in a setting with side information on the QM9 dataset which contains the chemical structures and properties of 134 kilo molecules \cite{rudd2012,rama2014}. As modern chemistry and material science are increasingly concerned with material property prediction, we show that \textit{DeepAA} can be used to \textit{systematically} explore vast chemical spaces in order to identify starting points for further chemical optimisation.
%
% screening methods to \textit{systematically} explore vast chemical spaces in %order to identify starting points for further chemical optimisation, become %indispensable. We show that \textit{DeepAA} is one such method.




%Screening methods seek to sample a vast chemical space in order to identify starting points for %further chemical optimisation. 

%material property prediction,

%Chemical space, taken here to mean the set of organic molecules of suitable size and composition to %potentially be oral drugs, is vast. 



%insights  properties structure

%molecules

%exploration

%Approximation. Trade off between interpretability and number of ATs.

==> 128-paper (2)/a02_deepAT_THEORY_gcpr2019.tex <==
\section{Method}
\label{sec_theo}
%In the following we will use \textit{linear} AA when referring to the original archetype model from \cite{cutlerBreiman1994}.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Linear Archetypal Analysis}
Linear AA \cite{cutlerBreiman1994} is a form of non-negative matrix factorization where a matrix $X\in \mathbb{R}^{n\times p}$ of $n$ data vectors is approximated as $X\approx ABX = AZ$ with $A\in \mathbb{R}^{n\times k}$, $B\in \mathbb{R}^{k\times n}$, and usually $k < \min\{n,p\}$. In AA parlance, the \textit{archetype} matrix $Z\in \mathbb{R}^{k\times p}$ contains the $k$ archetypes $\mathbf{z}_1,..,\mathbf{z}_j,.., \mathbf{z}_k$ and the model is subject to the following constraints:
%In theory a perfect decomposition is obtained for $BA = I_{n\times n}$.
%The following constraints on $A$ and $B$ give the rows $\mathbf{z}_j$ their %meaning and make linear Archetypal Analysis highly interpretable:
%
\begin{equation}\label{eq:constraint_A_B}
a_{ij} \geq 0 \text{ }\wedge\text{ } \sum_{j=1}^{k} a_{ij} = 1, \quad 
b_{ji} \geq 0 \text{ }\wedge\text{ } \sum_{i=1}^{n} b_{ji} = 1
\end{equation}
%
Constraining the entries of $A$ and $B$ to be non-negative and demanding that both weight matrices are row stochastic, implies a representation of the data vectors $\mathbf{x}_{i=1..n}$ as a weighted sum of the rows of $Z$ while simultaneously representing the archetypes $\mathbf{z}_{j=1..k}$ themselves as a weighted sum of the $n$ data vectors in $X$:
%
\begin{equation} \label{eq:at_decomp}
\mathbf{x}_i \approx \sum_{j=1}^{k} a_{ij} \mathbf{z}_j = \mathbf{a}_i Z, \quad
\mathbf{z}_j = \sum_{i=1}^{n} b_{ji} \mathbf{x}_i  = \mathbf{b}_j X
\end{equation}
%
Due to the constraints on $A$ and $B$ in Eq. \ref{eq:constraint_A_B} both the representation of $\mathbf{x}_i$ and $\mathbf{z}_j$ in Eq. \ref{eq:at_decomp} are \textit{convex} combinations. Therefore the archetypes approximate the data convex hull and increasing the number $k$ of archetypes improves this approximation. The central problem of AA is finding the weight matrices $A$ and $B$ for a given data matrix $X$.

A probabilistic formulation of linear AA is provided in \cite{seth2016} where it is observed that AA follows a simplex latent variable model and normal observation model. The generative process for the observations $\mathbf{x}_i$ in the presence of $k$ archetypes with archetype weights $\textbf{a}_i$ is given by
%
\begin{equation}\label{eq:probAT_1}
\mathbf{a}_i \sim \text{Dir}_k(\boldsymbol{\alpha}) \quad \text{ }\wedge\text{ } \quad
\mathbf{x}_i \sim \mathcal{N}(\mathbf{a}_iZ,\,\epsilon^2 \mathbf{I}),
\end{equation}
%
with uniform concentration parameters $\alpha_j = \alpha$ for all $j$ summing up to $\mathbf{1}^\top\boldsymbol{\alpha}=1$. That is the observations $\mathbf{x}_i$ are distributed according to an isotropic Gaussian with means $\boldsymbol{\mu}_i=\mathbf{a}_iZ$ and variance $\epsilon^2$. 

% In \cite{cutlerBreiman1994} an alternating least squares approach is proposed %to minimize the approximation error $E = \left\lVert X-ABX \right\rVert^2$.\\

%Archetypal Analysis describes a data set as a weighted mixture of extreme %points as each data point $\mathbf{x}_i$ is described as a convex mixture of %the archetypes $\mathbf{z}_{j=1..k}$. 



%Interpretability in the sense of Archetypal Analysis arises through the weight %vectors $\mathbf{a}_{i=1..n}$ in Eq. \ref{eq:at_decomp}: Each data point $%\mathbf{x}_i$ is described as a convex mixture of the archetypes $\mathbf{z}%_{j=1..k}$ which are considered pure (or extreme) points of the data. Thus %Archetypal Analysis describes a data set as a weighted mixture of extreme %points in contrast to clustering models where the most typical data points %(prototypes) are used to provide a lower dimensional representation of the data.



%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Deep Variational Information Bottleneck}
We propose a model to generalise linear AA to the non-linear case based on the Deep Variational Information Bottleneck framework since it allows to incorporate side information $Y$ by design and is known to be equivalent to the VAE in the case of $Y=X$, as shown in \cite{alemi2016}. In contrast to the data matrix $X$ in linear AA, a non-linear transformation $f(X)$ giving rise to a latent representation $T$ of the data suitable for (non-linear) archetypal analysis is considered. I.e. the latent representation $T$ takes the role of the data $X$ in the previous treatment.\\
The DVIB combines the information bottleneck (IB) with the VAE approach \cite{tishby2000,kingmaWelling2013}. The objective of the IB method is to find a random variable $T$ which, while compressing a given random vector $X$, preserves as much information about a second given random vector $Y$. The objective function of the IB is as follows
%
\begin{equation}
\mbox{min}_{p(\mathbf{t}|\mathbf{x})} I(X;T) - \lambda I(T;Y),
\label{eq:ib1}
\end{equation}
%
where $\lambda$ is a Lagrange multiplier and $I$ denotes the mutual information. Assuming the IB Markov chain $T-X-Y$ and a parametric form of Eq. \ref{eq:ib1} with parametric conditionals $p_\phi(\mathbf{t}|\mathbf{x})$ and $p_\theta(\mathbf{y}|\mathbf{t})$, Eq. \ref{eq:ib1} is written as
%
\begin{equation}
\max_{\phi,\theta}  -I_{\phi}(\mathbf{t};\mathbf{x}) + \lambda  I_{\phi,\theta}(\mathbf{t};\mathbf{y}).
\label{eq:ib_parametricForm}
\end{equation}
%
As derived in \cite{2018arXiv180406216W}, the two terms in Eq. \ref{eq:ib_parametricForm} have the following forms:
%
\begin{equation}
\label{eq:encoder_parametric}
I_{\phi}(T;X) = D_{KL}\left( p_\phi(\mathbf{t}|\mathbf{x}) p(\mathbf{x}) \| p(\mathbf{t}) p(\mathbf{x})\right) = \mathbb{E}_{p(\mathbf{x})}  D_{KL}\left(p_\phi(\mathbf{t}|\mathbf{x})\| p(\mathbf{t}) \right)
\end{equation}
%
and
%
\begin{equation}
\label{eq:decoder_parametric}
\begin{aligned}
I_{\phi,\theta}(T;Y) &=\ D_{KL}\left(\left[\int p(\mathbf{t}|\mathbf{y},\mathbf{x})p(\mathbf{y},\mathbf{x})\, \mathrm{d}\mathbf{x} \right] \| p(\mathbf{t}) p(\mathbf{y})\right)\\
&=\ \mathbb{E}_{p(\mathbf{x},\mathbf{y})} \mathbb{E}_{p_\phi(\mathbf{t}|\mathbf{x})}\log p_\theta(\mathbf{y}|\mathbf{t}) + h(Y).
\end{aligned}
\end{equation}
Here $h(Y)=-\mathbb{E}_{p(\mathbf{y})}\log p(\mathbf{y})$ denotes the entropy of $Y$ in the discrete case or the differential entropy in the continuous case. The models in Eq. \ref{eq:encoder_parametric} and Eq. \ref{eq:decoder_parametric} can be viewed as the encoder and decoder, respectively. Assuming a standard prior of the form $p(\mathbf{t})=\mathcal{N}(\mathbf{t};0,I)$ and a Gaussian distribution for the posterior $p_\phi(\mathbf{t}|\mathbf{x})$, the KL divergence in Eq. \ref{eq:encoder_parametric} becomes a KL divergence between two Gaussian distributions which can be expressed in analytical form as in \cite{kingmaWelling2013}. $I_\phi(T;X)$ can then be estimated on mini-batches of size $m$ as 
%
\begin{equation}
\label{eq:vae_encoder}
I_\phi(\mathbf{t};\mathbf{x}) \approx \frac1m \sum_i D_{KL}\left(p_\phi(\mathbf{t}|\mathbf{x}_i)\| p(\mathbf{t}) \right).
\end{equation}
%
As for the decoder, $\mathbb{E}_{p(\mathbf{x},\mathbf{y})} \mathbb{E}_{p_\phi(\mathbf{t}|\mathbf{x})}\log p_\theta(\mathbf{y}|\mathbf{t})$ in Eq. \ref{eq:decoder_parametric} is estimated using the reparametrisation trick proposed by  \cite{kingmaWelling2013,rezende2014}: 
\begin{equation}
\label{eq:vae_decoder}
I_{\phi,\theta}(\mathbf{t};\mathbf{y}) = \mathbb{E}_{p(\mathbf{x},\mathbf{y})} \mathbb{E}_{\boldsymbol{\varepsilon} \sim \mathcal{N}(0,I)} \sum_i  \log  p_{\theta}\left(\mathbf{y}_i|\mathbf{t}_i = \boldsymbol{\mu}_{i}(\mathbf{x}) + diag\left(\boldsymbol{\sigma}_i(\mathbf{x})\right) \boldsymbol{\varepsilon}\right) +\mbox{const.}
\end{equation}
%
Note that without loss of generality we can assume $Y=(Y',X)$ in Eq. \ref{eq:ib_parametricForm} and with $Y=X$ the original VAE is retrieved. The former will be used in the section \ref{subsec_ChemVAE} experiment where side information $Y'$ is available.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Deep Archetypal Analysis}
Deep Archetypal Analysis can then be formulated in the following way. For the sampling of $\mathbf{t}_i$ in Eq. \eqref{eq:vae_decoder} the probabilistic AA approach as in Eq. \eqref{eq:probAT_1} can be used which leads to
%
\begin{equation}
\label{eq:deepAA_t}
\mathbf{t}_i \sim \mathcal{N}\left(\boldsymbol{\mu}_i(\mathbf{x})=\mathbf{a}_iZ,\,\boldsymbol{\sigma}_i^2(\mathbf{x}) \mathbf{I}\right),
\end{equation}
%
where the mean $\boldsymbol{\mu}_i$ given through $\mathbf{a}_i$ and variance $\boldsymbol{\sigma}_i^2$ are non-linear transformations of the data point $\mathbf{x}_i$ learned by the encoder. We note that the means $\boldsymbol{\mu}_i$ are convex combinations of weight vectors $\mathbf{a}_i$ and the archetypes $\mathbf{z}_{j=1..k}$ which in return are considered to be convex combinations of the means $\boldsymbol{\mu}_{i=1..m}$ and weight vectors $\mathbf{b}_j$.\footnote{Note that $i=1..m$ (and not up to $n$), which reflects that deep neural networks usually require batch-wise training with batch size $m$.} By learning weight matrices $A\in \mathbb{R}^{m\times k}$ and $B\in \mathbb{R}^{k\times m}$ which are subject to the constraints formulated in Eq. \eqref{eq:constraint_A_B} and parameterised by $\phi$, a non-linear transformation of data $X$ is learned which drives the structure of the latent space to form archetypes whose convex combination yield the transformed data points. A major difference to linear AA is that for \textit{DeepAA} we cannot identify the positions of the archetypes $\mathbf{z}_j$ as there is no absolute frame of reference in latent space. We thus position $k$ archetypes at the vertex points of a $(k-1)$-simplex and collect these \textit{fixed} coordinates in the matrix $Z^{\text{fixed}}$. These requirements lead to an additional archetypal loss of
%
\begin{equation}\label{eq:lossAT}
\ell_{\text{AT}} = ||Z^{\text{fixed}}-BAZ^{\text{fixed}}||_2^2 = ||Z^{\text{fixed}}-Z^{\text{pred}}||_2^2,
\end{equation}
%
where $Z^\text{pred} = BAZ^{\text{fixed}}$ are the \textit{predicted} archetype positions given the learned weight matrices $A$ and $B$. For $Z^\text{pred}\approx Z^\text{fixed}$ the loss function $\ell_{\text{AT}}$ is minimized and the desired archetypal structure is achieved. The objective function of \textit{DeepAA} is then given by 
%
%{\color{red}{where $Z^\text{pred} = BAZ^{\text{fixed}}$ are the \textit{predicted} archetype positions given by the convex hull of the transformed data point %means $\mu$ during training. Minimizing $\ell_{\text{AT}}$ achieves the desired archetypal structure in latent space.}} 
%
\begin{equation}
\max_{\phi,\theta}  -I_{\phi}(\mathbf{t};\mathbf{x}) + \lambda  I_{\phi,\theta}(\mathbf{t};\mathbf{y})-\ell_{\text{AT}}.
\label{eq:ib_DeepAA}
\end{equation}
%
A visual illustration of \textit{DeepAA} is given in Fig. \ref{fig:at-supervised-arch}. The constraints on $A$ and $B$ can be guaranteed by using softmax layers and \textit{DeepAA} can be trained with a standard stochastic gradient descent technique such as Adam \cite{KingmaB14}.

%%which leads to a new loss function we call \textit{Archetype Loss}, AT-loss for short.
%
%%\begin{equation}\label{eq:lossAT}
%%\ell_{\text{AT}} = ||Z^{\text{f}}-BM||_F^2
%%\end{equation}
%

%\subsection{Implementation Details}
%We force the constraints in Eq. \ref{eq:constrained_ib_parametricForm} by implementing a new loss function we call \textit{Archetype Loss}, AT-loss for short:
%%
%\begin{equation}\label{eq:lossAT}
%\text{loss}_{\text{AT}} = ||\mu^{\text{dir}}-\mu^{\text{pred}}||_F^2 + ||Z^{\text{fixed}}-Z^{\text{pred}}||_F^2
%\end{equation}
%%
%The model architecture is shown in Fig. \ref{fig:at-supervised-arch}. From the last layer of the encoder we learn $A_{\mu}$, $B_z$, $\mu^{\text{direct}}$ and the variance. The AT-loss ensures that the predicted archetypes $Z^{\text{pred}}$ as convex mixtures of the latent means $\mu^{\text{dir}}$ are mapped close to the coordinates defined in the matrix $Z^{\text{fixed}}$ (analog for $\mu^{\text{dir}}$). As a result the weight matrices $A$ and $B$ are estimated. In general, the archetype loss can be small only if input data is mapped closely to the fixed archetypes. One can regard the branch in Fig. \ref{fig:at-supervised-arch} containing $\mu^{\text{direct}}$ and the variance as a vanilla VAE with an \textit{additional} contraint given by the AT-loss and the branch containing $A_{\mu}$ and $B_z$. In Fig. \ref{fig:trainingSeqMNIST} we show the 2-dim latent space for the popular MNIST digits \cite{lecunmnist} during training (4 leftmost panels). The three archetypes, mapped into the corners of the simplex, are `0', `1' and `7'\footnote{A detailed implementation is provided in case of acceptance. http...}.
%
\begin{figure}[h]
\begin{center}
   %\includegraphics[scale=.60]{arch_super_new}
%   \includegraphics[scale=.75]{arch_at_vae}
   \includegraphics[scale=.48]{Illustration_deepAA.png}
   
\end{center}
   \caption{Illustration of the \textit{DeepAA} model. \textbf{Encoder side}: Learning weight matrices $A$ and $B$ allows to compute the archetype loss $\ell_{AT}$ in Eq. \eqref{eq:lossAT} and sample latent variables $\mathbf{t}$ as described in Eq. \eqref{eq:deepAA_t}. The constraints on $A$ and $B$ in Eq. \eqref{eq:constraint_A_B} are enforced by using softmax layers. \textbf{Decoder side}: $Z^\text{fixed}$ represent the fixed archetype positions in latent space while $Z^\text{pred}$ are given by the convex hull of the transformed data point means $\mu$ during training. Minimizing $\ell_{AT}$ corresponds to minimizing the red dashed (pairwise) distances. The input is reconstructed from the latent variable $\mathbf{t}$. In the presence of side information, the latent representation allows to reproduce the side information $Y'$ as well as the input $X$.}
\label{fig:at-supervised-arch}
\end{figure}
%
%\begin{figure}[h]
%\begin{center}
%   \includegraphics[scale=.68]{trainingSeqMNIST}
%\end{center}
%	\caption{Latent space simplex during training of \textit{DeepAA} on MNIST after 1, 2, 60 and 300 epochs (from left to right.) The two rightmost figures show pathological cases. In the first of the two cases, the influence of the Archetype Loss was too high (with the divergence set too low) so that the inner of the simplex remains mostly unpopulated. In the second (rightmost) case, the Archetype Loss was too high while the divergence was kept at the same level as in the training of \textit{DeepAA} that produced the first four images.}
%\label{fig:trainingSeqMNIST}
%\end{figure}
%
%Latent space simplex during training of the DeepAA-VAE on MNIST after 1,
%2, 60 and 300 epochs (from left to right.) The two rightmost figures
%show pathological cases. In the first of the two cases, the influence of
%the Archetype Loss was too high (with the divergence set too low) so
%that the inner of the simplex remains mostly unpopulated. In the second
%(rightmost) case, the Archetype Loss was too high while the divergence
%was kept at the same level as in the training of the DeepAA-VAE that
%produced the first four images.
%
%\caption{Training a AT-VAE on MNIST. From left: After 1, 2, 60 and 300 Epochs. The two %rightmost figures show pathgological cases where the influence of the Archetype loss was too %high (with the divergence set too low) so that the inner of the simplex remains mostly %unpopulated or with AT loss too high but Divergence kept at the same level as for training %the AT-VAE that produced the first four images.}
%
%From a probabilistic viewpoint, linear AA can be seen as a linear latent variable model where the observations $\mathbf{x}_i$ are described as convex mixtures of the rows of the archetype matrix $Z$ (Eq. \ref{eq:at_decomp}) and scattered around the means $\mathbf{a}_iZ$ according to isotropic Gaussian noise with variance $\epsilon$. With the mixing components $a_{ij}$ summing to one (Eq. \ref{eq:constraint_A_B}), we formalize these relations as follows
%%
%\begin{equation}\label{eq:probAT_1}
%\mathbf{a}_i \sim \text{Dir}_k(\boldsymbol{\alpha}) \quad \text{ }\wedge\text{ } \quad
%\mathbf{x}_i \sim \mathcal{N}(\mathbf{a}_iZ,\,\epsilon \mathbf{I}),
%\end{equation}
%%
%with $\sum_{j=1}^k\alpha_j = \mathbf{1}^t\boldsymbol{\alpha}=1$. But linear AA also needs archetypes to be convex mixtures of the data, which leads to the following:
%%
%\begin{equation}\label{eq:probAT_2}
%\mathbf{b}_j \sim \text{Dir}_k(\boldsymbol{\beta}) \quad \text{ }\wedge\text{ } \quad
%\mathbf{z}_j \sim \mathcal{N}(\mathbf{b}_jX,\,\epsilon \mathbf{I}),
%\end{equation}
%%
%with $\sum_{i=1}^n\beta_i = \mathbf{1}^t\boldsymbol{\beta}=1$. Thus, the log-likelihood can be written as:
%%
%\begin{multline}\label{eq:AT_loglik}
%\text{log}\mathcal{L}(X|B,A,X,Z) = \\ -\frac{\epsilon}{2}||X-AZ||_F^2 - \frac{\epsilon}{2}||Z-BX||_F^2+C(\epsilon)
%\end{multline}
%%
%Under the constraints given by Eq. \ref{eq:constraint_A_B}, the archetype matrix $Z$ and corresponding weights $A$ are found by 
%
%
%
%
%\newpage
%
%
%%Approximation. Trade off between interpretability and number of ATs.
%\paragraph{Unsupervised} Our approach is based on the variational autoencoder (VAE) framework proposed by \cite{kingmaWelling2013, rezende2014} where latent variables $\latZ$ are generatedArchetypal Analysis requires the means $\boldsymbol{\mu}_j$ in Eq. \ref{eq:probAT_1}, i.e. the latent samples in \textit{DeepAA}, to be convex combinations of the archetypes $\mathbf{z}_j$. But at the same time the archetypes $\mathbf{z}_j$ need to be convex mixtures of the means $\boldsymbol{\mu}_j$. Following \cite{seth2016}, the generative process for the observations $\mathbf{t}_i$ is as follows:
%
%\begin{equation}\label{eq:probAT_1}
%\mathbf{a}_i \sim \text{Dir}_k(\boldsymbol{\alpha}) \quad \text{ }\wedge\text{ } \quad
%\mathbf{t}_i \sim \mathcal{N}(\underbrace{\mathbf{a}_iZ}_{\boldsymbol{\mu}_i},\,\epsilon^2 \mathbf{I}),
%\end{equation}
%%
%with $\sum_{j=1}^k\alpha_j = \mathbf{1}^t\boldsymbol{\alpha}=1$. The $\mathbf{a}_i$ are the weights of the archetypes while the observations $\mathbf{t}_i$ are scattered around the means $\boldsymbol{\mu}_i=\mathbf{a}_iZ$ according to isotropic Gaussian noise with variance $\epsilon^2$.\\
%% from a prior distribution $p_\theta(\latZ)$. The data $\mathbf{x}$ is then generated by the decoder $p_\theta(\mathbf{x}|\latZ)$ conditioned on $\latZ$. For estimating the parameters $\theta, \phi$ of such a model, \cite{kingmaWelling2013} introduces a stochastic gradient variational Bayes method where the variational bound $\mathcal{L}(\mathbf{x};\theta,\phi)$ of the log-likelihood $p_\theta(\mathbf{x})$ is maximized:
%%
%\begin{eqnarray}
%\label{eq:logLikelihood}
%p_\theta(\mathbf{x}) &=& D_{KL}(q_\phi(\latZ|\mathbf{x})|| p_\theta(\latZ|\mathbf{x})) + \mathcal{L}(\mathbf{x};\theta,\phi) \\
%\label{eq:elbo}
%p_\theta(\mathbf{x}) &\geq& \mathcal{L}(\mathbf{x};\theta,\phi) = \notag \\
%&& \mathbb{E}_{q_\phi(\latZ|\mathbf{x})}[-\log q_\phi(\latZ|\mathbf{x}) + \log p_\theta(\mathbf{x,\latZ})]
%\end{eqnarray}
%%
%The distribution $q_\phi(\latZ|\mathbf{x})$, also known as the encoder, is an approximation to the true posterior $p_\theta(\latZ|\mathbf{x})$. Here, both encoder and decoder are parametrized by neural networks and posterior and latent variables $\latZ$ are assumed to be Gaussian.
%%
%\begin{figure}[h]
%\begin{center}
%   \includegraphics[scale=.60]{arch_super_3}
%\end{center}
%   \caption{DeepAA-VAE, Encoder: Weight Matrices $A_\mu$ and $B_z$ are learned in tandem as minimizing the archetype loss is equivalent to finding a representation of the indentity matrix as $I^{k\times k} = B_zA_\mu$. Means $\boldsymbol{\mu}$ and variances $\sigma$ are generated by the encoder so that implementing archetype loss requires modifiying only the encoder part of a VAE.}
%\label{fig:at-supervised-arch}
%\end{figure}
%%
%In linear AA archetypes $\mathbf{z}_j$ are linear combinations of features and finding the matrix $Z$ implies learning their positions in feature space. This cannot not hold true for latent variable models like VAEs where the input data is mapped into latent space by arbitrarily complex, non-linear functions. As a consequence, latent coordinates hold no absolute meaning and thus learning their positions is nonsensical. We therefore propose to designate $k$ archetype positions in a $k-1$-dimensional latent space as the corners of a $(k-1)$-simplex whose center coincides with the origin of the latent space coordinate system. These positions are given by the constant matrix $Z^{\text{fixed}}$. To ensure a bijective mapping between latent space coordinates $\latZ^{(i)} = (z^{(\mathscr{l})}_{i1},..,z^{(\mathscr{l})}_{i,k-1})^T$ and barycentric coordinates, i.e. coordinates expressed by mixture coefficients $\mathbf{a}_i = a_{i1},..,a_{ik}$ relative to $Z^{\text{fixed}}$, we need to open up a new latent dimension for each additional archetype. Analogous to linear AA,
%%
%\newpage
%\paragraph{Supervised}
%%
%our goal is to learn latent mixture matrices $A_\mu$ and $B_z$ such that the latent means $\boldsymbol{\mu}_i$ can be written as a convex mixture of the archetypes, i.e. $\boldsymbol{\mu} = A_\mu Z^{\text{fixed}}$ while the archetypes are represented as a convex mixture of the data $Z^{\text{fixed}} = B_z \boldsymbol{\mu}$. For an input datum $\mathbf{x}_i$ the corresponding latent coordinates $\boldsymbol{\mu}_i$ are the product of the mixture coefficients and the fixed archetype matrix $Z^{\text{fixed}}$
%\begin{equation}
%\boldsymbol{\mu}_i = (a_{i1},..,a_{ik}) \cdot Z^{\text{fixed}}.
%\end{equation}
%Thus when training our VAE the latent means $\boldsymbol{\mu}_i$ are learned only indirectly by learning the mixture weights $A_\mu$ of the latent means. Learning the weight matrix $B_z$ of the latent archetypes is slightly more involved: As we use the same layer of our encoding network to provide the weight matrix $A_\mu\in \mathbb{R}^{n\times k}$ and $B_z\in \mathbb{R}^{k\times n}$ with dimensions reversed, we simply learn the transpose $B_z^T$ and apply a transpose and softmax operation on the learned $B_z^T$. Finally, we obtain the row-stochastic weigth matrix $B_z$ so that the archetypes, expressed as a convex mixture of the latent $\mu$'s, are given by the product $B_z\cdot \mu$. We now introduce a new loss function, the so called Archetype Loss, by translating the convexity constrained linear combinations from linear AA shown in Eq. \ref{eq:at_decomp} into the following expressions:
%
%\begin{eqnarray}
%\label{comb1}
%\boldsymbol{\mu} &=& A_\mu Z^{\text{fixed}} \\
%\label{comb2}
%Z^{\text{predicted}} &=& B \boldsymbol{\mu}
%\end{eqnarray}
%
%We use the fact that the latent archetypes themselves are mixtures of the latent means to obtain a prediction $Z^{\text{predicted}}$ of the actual archetypes at every training iteration. Measuring the difference between this prediction and the desired positions of the archetypes given by $Z^{\text{fixed}}$ allows us to formulate the following loss function
%
%\begin{equation}
%\label{eq:z_pred}
%Z^{\text{predicted}} = B_z A_\mu Z^{\text{fixed}}
%\end{equation}
%
%which simply results from inserting Eq. \ref{comb1} into Eq. \ref{comb2}. Finally we can write the Archetype Loss as:
%
%\begin{equation}
%\label{at_loss}
%\text{AT Loss} = ||Z^{\text{fixed}} - Z^{\text{predicted}}||_2
%\end{equation}
%
%A formal difference to the linear AA model can be seen in Eq. \ref{eq:z_pred} where equality bewteen $Z^{\text{predicted}}$ and $Z^{\text{fixed}}$ is obtained for $B_z A_\mu = I^{k\times k}$. In linear AA the approximation $X\approx ABX$ is optimal for $A B = I^{n\times n}$ where the rank of $B$ is at most $k$ \cite{Bauckhage2014}. The modifications involved in extending a standard variational (Gaussian) autoencoder to become an archetype autoencoder (AT-VAE) are given in Fig. \ref{fig:at-vae}. Necessary changes are minor and only involve the encoder \footnote{code will be provided}. Most importantly, while learning the mixture matrices $A_\mu$ and $B_z$ in order to calculate the AT Loss, the encoder will output latent means $\boldsymbol{\mu}_i$ and variances $\sigma_i$ so that latent samples $\latZ^{(i)} = \boldsymbol{\mu}_i(X)+\epsilon\cdot\sigma_i^{1/2}(X)$ can be generated in the usual way and the reparametrization trick remains unaffected by the archetype extension.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\paragraph{Parameter Selection} We propose to extend the unsupervised AT-VAE model described in the previous section to incorporate (partial) label information. This extension is based on the idea of the information bottleneck (IB) proposed in \cite{tishby2000} the deep variational information bottleneck (DVIB) proposed in \cite{alemi2016}. The idea of the IB is to compress a random variable $x$ while retaining as much information as possible about a second variable $y$. This can be formulated as the following variational problem formualted using mutual information $I(\cdot;\cdot)$
%\begin{equation}
%\min_{p(t|x)}I(x;t) - \lambda I(t;y)
%\label{ibVar}
%\end{equation}
%where it is assumed that $y$ is conditionally independent of $t$ given $x$. Combining the idea of IB and VAE  
%
%
%
%\begin{itemize}
%\item theory: info curves, infoBottleneck
%\item model selection: how many ATs
%\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% (107)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\paragraph{Parameter Selection} When training a AT-VAE two additional parameters need to be chosen which are the number of archetypes and the prefactor or weight of the AT loss relative to the likelihood and the divergence. The first parameter, the number of archetypes, depends on how many factors of variation of approximately equal importance are represented in the dataset: If a prominent factor of variation like the different poses of a face is present, then a smaller factor like 'wearing eye glasses' is much more likely to be placed inbetween two archetypes than forming an archetype on its own. As a consequence we suggest selecting archetypes in the low two digit numbers. Furthermore, as each new archetype requires a new latent dimension, the amount of available training data might play role as well. We have observed that for high numbers of archetypes only mean reconstructions similar to the one in Fig. \ref{fig:at_mean} (middle) appear. It would thus be possible to implement a dissimilarity score to measure the diversity of archetypes and use this score to select the number of archetypes associated with the peak of that score. But this would beg the question of how to measure dissimilarity in the respective domains under consideration. We therefore rely on visual inspection of the archetypes for our experiments on CelebA.
%
%\begin{figure}[h]
%\begin{center}
%   \includegraphics[scale=.68]{trainingSeqMNIST}
%\end{center}
%	\caption{Training a AT-VAE on MNIST. From left: After 1, 2, 60 and 300 Epochs. The two rightmost figures show pathgological cases where the influence of the Archetype loss was too high (with the divergence set too low) so that the inner of the simplex remains mostly unpopulated or with AT loss too high but Divergence kept at the same level as for training the AT-VAE that produced the first four images.}
%\label{fig:trainingSeqMNIST}
%\end{figure}
%
%The second parameter, the weight of the archetype loss, should be selected as small as possible. The latent space during training of a AT-VAE on MNIST is shown in Fig. \ref{fig:trainingSeqMNIST}. With a small prefactor of the AT loss, divergence and likelihood will dominate the first stages of training and the simplex, which represents a local minimum, is overlooked at first. This is important, as -- while the latent structure is forming -- the latent means will gradually retreat into the simplex leaving the more diverse or archetypal points close to the corners of the simplex whereas points associated with more similar reconstructions will proceed further into the direction of the origin. This process can be observed in the first three panels of Fig. \ref{fig:trainingSeqMNIST}. In conjunction with the AT loss a sensitive hyperparameter to be tuned is the prefactor of the divergence: Assuming a AT-VAE with Gaussian prior it is clear that the simplex, being a non-sperical geometry, cannot produce a minimal KL-Divergence and a minimum AT loss at the same time. %On the other hand does the Gaussian prior allow for relatively uniform starting conditions
%Fortunately the divergence prefactor can be automatically tuned for a given number of archetypes. The procedure is as follows:
%
%\begin{algorithm}
%\caption{Tuning prefactor of $D_{\text{KL}}$ for AT-VAE}
%\begin{algorithmic}
%\REQUIRE $n \geq 0 \vee x \neq 0$
%\ENSURE $y = x^n$
%\STATE $y \leftarrow 1$
%
%\WHILE{$N \neq 0$}
%\IF{$N$ is even}
%\STATE $X \leftarrow X \times X$
%\STATE $N \leftarrow N / 2$
%\ELSE[$N$ is odd]
%\STATE $y \leftarrow y \times X$
%\STATE $N \leftarrow N - 1$
%\ENDIF
%\ENDWHILE
%\end{algorithmic}
%\end{algorithm}
%
%%\begin{itemize}
%%\item latent convex mixture
%%\item effect of AT loss, number of ATs
%%\item optimal AT vs non-opt AT (relation to disentanglement)
%%\item what happens when going to high dims, why should one not...
%%\item what prior to use...
%%\item why number of ATs is connected to number of dimensions (uniqueness!, vs %GMM)
%%\end{itemize}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\paragraph{Effect of Archetype Loss} Variational autoencoders have shown the ability to interpolate by establishing semantically meaningful variations for reconstucted images whose latent representations are in close proximity to each other. This ability has its roots in the randomness inherent to the training procedure of VAEs but is not explicitly enforced. This can be seen in the objective function given in Eq. \ref{eq:elbo}, which contains no reference to pairwise dependences between samples $\latZ^{(i)}$ and $\latZ^{(j)}$. The archetype loss introduces, through the mixtures matrices $A_\mu$ and $B_z$, an explicit and very specific relation between latent variables $\latZ$ and therefore by extension a relation between reconstructed data points: Data points that are highly dissimilar have a high probability for their latent representations to be located far apart from each other. As we assume an equidistant simplex, where the furthest distance possible is the distance between any two corners of the simplex, the reconstructed data points whose latent means are close to the corners will usually exhibit the highest perceived degree of variability. Furthermore latent points $\latZ$ located in proximity to the centre of the simplex, i.e. located at equal distances from each corner, are associated with reconstructed inputs that share an equal degree of similarity with each of the archetypes -- in this sense these data points represent averages of the whole dataset as shown in Fig \ref{fig:at_mean}.
%
%\begin{figure}[h]
%\begin{center}
%   \includegraphics[scale=1.0]{at_mean}
%\end{center}
%   \caption{From left: Samples taken at the position of (1) an archetype, (2) the origin and (3) another archetype for a AT-VAE trained on CelebA. The reconstructed image sampled from the origin appears female and reflects the bias or class imbalance towards females (58.3\%) vs males (41.7\%) with an image total of 202,599.}
%\label{fig:at_mean}
%\end{figure}
%
%Archetype loss introduces an interpretable, global structure into latent space that gives meaning to distances and directions relative to the barycentric coordinate system spanned by the archetypes. But introducing a loss that depends on the relation between data points implies a lower limit to the size of a minibatch which should contain no less than $k$ samples where $k$ is the number of archetypes to be learned.


==> 128-paper (2)/a03_deepAT_EXPERIMENTS_Artificial_gcpr2019.tex <==
\section{Experiments}
\label{sec_exp}
%
\subsection{Artificial Experiments}
\label{subsec_artificial}
%
\subsubsection{Data generation}
%
For our experiments we generate data $\mathbf{X}\in \mathbb{R}^{n\times 8}$ that are a convex mixture of $k$ archetypes $\mathbf{Z}\in \mathbb{R}^{k\times 8}$ with $k\ll n$. The generative process for the data $\mathbf{x_i}$ follows Eq. \eqref{eq:probAT_1} where $\mathbf{a}_i$ are stochastic weight vectors denoting the fraction of each of the $k$ archetypes $\mathbf{z}_j$ needed to represent the data point $\mathbf{x}_i$. Here, we generate $n=10000$ data points of which $k=3$ are true archetypes. We set the variance to $\sigma^2=0.05$. We embed our linear 3-dim data manifolfd in a $n=8$ dimensional space. Note that although classical and deep archetypal analysis is always performed on the full data set we only use a fraction of the data when visualizing our results.
%
%
\subsubsection{Linear archetypal analysis -- linear data}
%
Linear archetypal analysis is performed using the efficient Frank-Wolfe procedure proposed in \cite{bauck2015FW}. The input data is 8-dimensional and consequently the dimensionality of the archetypes is $\mathbf{Z}\in \mathbb{R}^{3\times 8}$. For visualization we then use PCA to recover the original 3-dimensional manifold. The first three principal components of the ground truth data are shown in Fig. \ref{fig:art1} as well as the computed archetypes (green triangles). The positions of the computed archetypes are in very good agreement with the ground truth.
%
\begin{figure}[h!]
	\begin{center}
		\includegraphics[scale=.3]{figs/classicAA_3AT_in_8dim.png}
	\end{center}
	\vspace{-1.8em}
	\caption{PCA projection of 8-dim data after performing linear archetypal analysis. The original linear data submanifold is a convex combination of 3 archetypes.}
	\label{fig:art1}
\end{figure}
In these experiments, the data generating process is known and the number of archetypes $k=3$ can be considered as an available \textit{side information}.
%Using data for which we know the generative process the true number $k=3$ of archetypes is known. Here $k=3$ is what we call the \textit{side information} used when performing archetypal analysis.
%In practice a suitable model would be selected by observing how an appropriate loss functions is changing in dependence of the number $k$ of archetypes used. %But large numbers of archetypes tend in general to make 
%
%
\subsubsection{Linear archetypal analysis -- non-linear data}
%
Introducing a non-linearity to the data, e.g. by applying the exponential to a dimension of $\mathbf{X}$, results in a curved data submanifold as shown in Fig. \ref{fig:curvedSubmanifold3ATs}.
%
\begin{figure}[h!]
  \begin{subfigure}[t]{.48\textwidth}
  \centering
    \includegraphics[width=.95\textwidth]{figs/nonLin_data_3_opt_lin_ats_B.png}
    \caption{A curved 2-dim manifold. None of the three archetypes identified by linear archetypal analysis can be interpreted as extremes.}
    \label{fig:curvedSubmanifold3ATs}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.48\textwidth}
  \centering
    \includegraphics[width=.95\textwidth]{figs/nonLin_data_5_opt_lin_ats.png}
    \caption{Linear archetypal analysis requires at least five archetypes to describe the data convex hull reasonably well.}
    \label{fig:curvedSubmanifold5ATs}
  \end{subfigure}
  \caption{While linear archetypal analysis is in general able to approximate the data convex hull given a large enough number of archetypes, their interpretation as extremal elements is in general not ensured.}
\end{figure}
%
For example ratios of power or field quantities are usually measured in decibels which is the logarithm of the these ratios. An exponentiation, i.e. introducing a strictly monotone transform, should in general not change which data points are identified as archetypes nor the number of archetypes necessary to obtain a given loss value. Fig. \ref{fig:curvedSubmanifold3ATs} demonstrates that linear archetypal analysis is unable to recover the true archetypes on the same dataset used in the previous experiment but \textit{after} a strictly monotone transform had been applied. Moreover to obtain a similar reconstruction loss as for the \textit{linear} submanifold at least 5 archetypes are necessary as can be seen in Fig. \ref{fig:curvedSubmanifold5ATs}. Although the additional two archetypes are necessary to better aprroximate the data convex hull it would be counter-intuitive to interpret them as \textit{extremes} of the dataset.
%
%
\subsubsection{Non-linear archetypal analysis -- non-linear data}
%
Deep archetypal analysis \textit{without explicit} side information is used to learn a latent linear archetypal representation. We consider as implicit side information the knowledge that 3 archetypes were used to generate our artificial non-linear data and therefore chose a 2-dim latent space. 
%
\begin{figure}[h!]
  \begin{subfigure}[t]{.48\textwidth}
  \centering
    \includegraphics[width=.95\textwidth]{figs/classicAA_3AT_in_8dim_nonlinear.png}
    \caption{The first three principal components of a non-linear 8-dim manifold. Despite the curvature only three \textit{true} archetypes exist.}
    \label{fig:deep_curvedSubmanifold3ATs}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.48\textwidth}
  \centering
    \includegraphics[width=1.00\textwidth]{figs/latentSpace_3AT_in_8dim_nonlinear.png}
    \caption{2-dim latent space learned by deep archetypal analysis. Side information used was the known number of archetypes.}
    \label{fig:deepLatentSpce3ATs}
  \end{subfigure}
  \caption{Deep archetypal analysis maps the archetypes from data space onto the vertices of the simplex and conserves the stripe pattern visible in the data space.}
\end{figure}
%
In Fig. \ref{fig:deep_curvedSubmanifold3ATs} the first three principal components of the 8-dim data are shown. Data points have been colored according to the third principal component. In Fig. \ref{fig:deepLatentSpce3ATs} the learned latent space shows that the archetypes A, B and C have been mapped to the appropriate vertices of the latent simplex. Moreover the sequence of color stripes shown in Fig. \ref{fig:deep_curvedSubmanifold3ATs} has correctly been mapped into latent space. Within the latent space data points are again described as convex linear combinations of the latent archetypes. Latent data points can also be reconstructed in the original data space through the learned decoder network. The network architecture used for this experiment was a simple feedforward network (2 layered encoder and decoder), training for 20 epochs with a batch size of 100 and a learning rate of 0.001.



==> 128-paper (2)/a03_deepAT_EXPERIMENTS_Bats_gcpr2019.tex <==
\subsection{Representation Learning for \textit{Microchiroptera}}
\label{subsec_deepBats}
%
Based on expert knowledge \textit{body mass} and \textit{wing aspect ratio} were chosen to be the two most important features relating to the \textit{dominant food habit} of Microchiroptera, see Fig. \ref{fig:bats138}. But \cite{norberg1987} have collected six additional measurements on each species. These are \textit{wing span, wing area, wing loading, tip length ratio, tip area ratio and tip shape index}. Arguably, more meaningful archetypes may be found by learning an appropriate representation based on \textit{all} available measurements. We use \textit{DeepAA} to learn such a representation. Our encoder is shown in Fig. \ref{fig:at-supervised-arch}. Both encoder and decoder are parametrized by two feed-forward neural networks with two hidden layers each. We train the VAE for 200 epochs (learning rate: $1\text{e-}3$, batch size: 60) in a side information setting with the \textit{dominant food habit} as the additional information. 
%
%Based on physical intuition it is sensible to assume that bats whose primary food source are other flying %animals have evolved to be more aerodynamical than bats living off plant material.
%
\begin{figure}[h!]
\begin{center}
   \includegraphics[scale=.385]{bats138_deep}
\end{center}
\vspace{-1.8em}
\caption{\textit{DeepAA} finds a organisation of species not unsimilar to linear AA: Insectivores and frugivores populate opposite ends of the Pareto front. But the interesting insight is the representation associated with the latent space ordering found by \textit{DeepAA}. While linear AA was forced to find the best possible representation in the space of \textit{Wing Aspect Ratio} and \textit{Body Mass}, \textit{DeepAA} was free to learn a representation which included two additional features, i.e. $Wing Loading$ and $Tip Shape Index$. Based on these features \textit{DeepAA} was able to learn a richer representation which is in much agreement with the finding of \cite{norberg1987}, as discussed in the paragraph \textit{Results and Discussion}.}
\label{fig:bats138_deep}
\end{figure}
%
%
%\caption{Phenospace of 138 species of Microchiroptera. The dominant food habit of each %species, and thereby the ability to procure this food source, is linked to the morphology of %the animals, e.g. a higher \textit{Wing Aspect Ratio} corresponds with the greater aerodynamic %efficiency needed to chase high flying insects. Archetypes are extreme types, optimized to %perform a single task. Proximity of a species to an archetype quantifies the level of %adaptation this species has undergone with respect to the archetypal task.}
%
%
In order to compare to the results based on linear AA, we choose the same number of archetypes as in Fig. \ref{fig:bats138}. The representation learned by \textit{DeepAA} is shown in Fig. \ref{fig:bats138_deep}. By running the latent \textit{Archetypes A, B} and \textit{C} through the decoder of our trained VAE we obtain three sets of eight \textit{generated} features. Each set represents the traits of an archetypal species in terms of the eight measures introduced by \cite{norberg1987}. For these three species we analyze by how much each feature changes. This allows us to deduce the most important measures characterizing the relation between \textit{food habit} and \textit{morphology}.
%
\begin{table}%[b!]
\caption{Characteristic traits of the archetypes identified in Fig. \ref{fig:bats138_deep} and the task each archetypal species is optimized to perform.}
\label{tbl_deep_traits}
\vskip 0.05in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Measure & importance & A & B & C \\
\midrule
total mass        & 35\% & med  & low & high \\
wing area         & 30\% & low  & med & high \\
wing loading      & 15\% & low  & med & high \\
wing span         & 10\% & low  & low & high \\
tip shape index   & 10\% & high & med & low \\
%tip length ratio  & -- & & & \\
%tip area ratio    & -- & & & \\
%ing aspect ratio & -- & & & \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%
\paragraph{Results and Discussion} Our results are shown in Table \ref{tbl_deep_traits}. For each measure we consider the largest relative change with respect to the archetypes and take the magnitude of these changes as a proxy for feature importance. Similar to Fig. \ref{fig:bats138}, we find that \textit{total mass} is the most important feature: The heavier a bat the more likely it is to be a frugivore -- a result consistent with linear AA. But in contrast to the linear case \textit{DeepAA} does not consider \textit{wing aspect ratio}. Instead \textit{wing area} and \textit{wing span} are deemed important. But as \textit{wing aspect ratio} is simply the square of the \textit{wing span} divided by the \textit{wing area}, one could argue that \textit{DeepAA} captures the influence of \textit{wing aspect ratio} nonetheless. 
A novel insight produced by \textit{DeepAA} is the importance of two additional features, namely \textit{wing loading} and \textit{tip shape index}. According to \cite{norberg1987}, as wing loading increases, the bat must fly faster and expend more energy, and the range of accessible flight behavior is reduced. As \textit{Archetype A} has low \textit{wing loading}, thereby enabling various flight behaviors, it makes sense that this archetype can accommodate the largest variation in food habits, i.e. frugivore, nectarivore, insectivore, pescivore, carnivore and sanguivore are all found in proximity to \textit{Archetype A}. Regarding \textit{tip shape index}, \cite{norberg1987} find that it is inversely correlated with flight speed. They further state that flight speed increases significantly with \textit{wing loading}. As shown in Table \ref{tbl_deep_traits}, this is exactly the inverse relation learned by \textit{DeepAA} -- high \textit{wing loading} and low \textit{tip shape index} for \textit{Archetype A} while the inverse is true for \textit{Archetype C}. The learned representation is thus in very good agreement with the various trade-offs found by \cite{norberg1987}. But \textit{DeepAA} did not only find a richer and arguably more meaningful representation than linear AA, it also learned the appropriate scaling when combining the different features. By contrast, in linear AA one had to know \textit{beforehand} that \textit{total mass} would need to enter the model logarithmically.


%Consitent with the observation/calc from norberg, tip is....

%, low flight speed is correlated with large wingtip shape index, I

%speed increased significantly with wing loading

%Mass-carrying ability will be linked most closely with wing loading. As wing loading
%increases, the bat must fly faster and expend more energy, and the range of accessible flight
%ehaviour is reduced until flight is no longer possible. Because they habitually fly with
%ubstantial loads, we expect carnivores to have relatively low wing loading. Large wingspan

==> 128-paper (2)/a03_deepAT_EXPERIMENTS_CelebA_gcpr2019.tex <==
\subsection{Generative Aspects and Model Selection}
\label{subsec_celebA}
%
\textit{DeepAA} allows to generate samples by specifying the mixture coefficients or proportions each archetype shall have in the make-up of a new sample. As a proof of concept, archetypal faces in the large-scale CelebFaces Attributes (CelebA) dataset \cite{celebA2015} are learned and new faces generated.\\
In our experiment we adopt the "Deep Feature Consistent Variational Autoencoder" proposed by \cite{dfc_vae} which makes use of a (feature) perceptual loss as the reconstruction loss.  In our implementation, we use the VAE-123 model of the original paper with the modification as depicted in Fig. \ref{fig:at-supervised-arch}. We train our model with the Adam optimizer \cite{KingmaB14} at a learning rate of $0.0005$ and we set the first moment decay rate to $\beta_1=0.5$. Training is performed with a batch size of 64 for 10 epochs and 90\%/10\% split of the dataset for training/testing. In the experiment, no side information was used. In order to identify the appropriate number of archetypes we propose a model selection technique similar to the ''elbow'' method by \cite{hart2015}: The (minimal) reconstruction loss for different numbers of archetypes, evaluated on the test set, is recorded as shown in Fig. \ref{fig:celebA_IC}. The optimal number of archetypes is considered to be the point where the curve starts converging, which in our case is at 35 archetypes (archetypal faces can be found in the supplement). Fig. \ref{fig:celebA_seq_images} displays an exemplary interpolation of generated faces: Starting at the latent coordinates which represent the face of a young man we move along a straight line in direction of a vertex point of the latent space simplex. While moving along this line we decode, at regular intervals, a total of six latent samples.
%
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.8\textwidth]{figs/celebA_sample-seq-1_AT-23_image-7.png}
	\caption{Interpolation sequence towards an archetype representing an old man: While approaching the archetype (archetype B3 in the supplement), characteristic features of the archetypal face are reinforced.}
	\label{fig:celebA_seq_images}
\end{figure}

==> 128-paper (2)/a03_deepAT_EXPERIMENTS_Molecules_gcpr2019.tex <==
%\begin{figure}[!h]
%	\begin{center}
%		\includegraphics[width=0.6\textwidth]{figs/celebA_IC_Maxima.png}
%		\caption{Reconstruction loss with varying number of archetypes. } 
%		\label{fig:celebA_IC}
%	\end{center}
%\end{figure}
%
%
%
%
%\begin{figure}[!h]
%\begin{center}
%\includegraphics[width=0.5\textwidth]{figs/qm9_selection.pdf}
%\caption{Test MAE with a varying number of archetypes.} 
%\label{fig:qm9selection}
%\end{center}
%\end{figure}
%
\begin{figure}[hb!]
	\begin{subfigure}[t]{.48\textwidth}
	\centering
		\includegraphics[width=1.0\textwidth]{figs/celebA_IC_Maxima.png}
		\caption{CelebA: Reconstruction loss with varying number of archetypes. } 
		\label{fig:celebA_IC}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{.48\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{figs/qm9_selection.pdf}
		\caption{QM9: Test MAE with a varying number of archetypes.} 
		\label{fig:qm9selection}
	\end{subfigure}
\caption{Model selection curves: reconstruction loss vs the number of archetypes.} 
\end{figure}
%
%
\begin{figure*}[!h]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/long_chain.pdf}
        \caption{}\label{figure:case1}
    \end{subfigure} \hspace{1cm}
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/same_weight.pdf}
        \caption{}\label{figure:case2}
    \end{subfigure}
    \caption{The panels illustrate a comparison between two archetypes where the labels represent the corresponding heat capacity. Here, the columns denote the molecules that are closest to the specific archetype and the rows are the archetypes. Panel (a) compares a long chain versus a short chain archetype. Panel (b) compares archetypal molecules with the same mass but different shapes.}
    \label{fig:comparisions}
\end{figure*}

\subsection{Exploring Chemical Spaces with Side Information}
\label{subsec_ChemVAE}
\textbf{Dataset:} As mentioned in the introduction, archetypal analysis lends itself to a distinctly evolutionary interpretation. Although this is certainly a more biological perspective, the basic principle can be transferred to other fields such as chemistry. In this experiment we explore the chemical space which is the space of all molecules that already exist or can be produced. As side information we use the \textit{heat capacity} $C_v$ which quantifies the amount of energy (in Joule) needed to increase 1 Mol of molecules by 1 K at constant volume. Here, a high $C_v$ is especially important for a huge number of applications such as thermal energy storage \cite{CABEZA20151106}. In our experiments, we use the QM9 dataset \cite{rama2014,rudd2012} which was calculated on ab initio DFT method based structures and properties of 134k organic molecules with up to nine atoms (C, O, N, or F), without counting hydrogen.
%
%
%        \begin{subfigure}{0.3\textwidth}
%        \centering
%        \includegraphics[width=\textwidth]{figs/different_weight.pdf}
%        \caption{}\label{figure:case3}
%    \end{subfigure}   
%
\begin{figure*}[!h]
\begin{center}
\includegraphics[width=0.9\textwidth]{figs/interpolation.pdf}
\caption{Interpolation between two archetypes produced by our model. The label denote the molecules' heat capacity. While we show only one example, the same results can also be observed for other archetype combinations.} 
\label{fig:interpolation}
\end{center}
\end{figure*}

\textbf{Set-up:} We extracted 204 features for every molecule by using the Chemistry Development Kit \cite{cdk}. The neural architectures used have 3 hidden layers with 1024, 512 and 256 neurons, respectively and ReLU activation functions. We train our model in a \textit{supervised} fashion, by reconstructing the molecule and the side information simultaneously. In Experiment 1, we continuously increase the number of latent dimensions to perform model selection. In Experiment 2 and 3, we fix the number of latent dimensions to 19 which corresponds to 20 archetypes. During training, we steadily increase the Lagrange multiplier $\lambda$ by 1.01 every 500 iterations. Our model is trained with the Adam optimizer \cite{KingmaB14} with an initial learning rate of 0.01. We decay the learning rate with an exponential decay by 0.95 every 10k iterations. In addition, we use a batch size of 2048 and train the model for 350k iterations. The dataset is divided in a training and test split of 90/10\%.

In \textbf{Experiment 1}, we asses the MAE error when varying the number of archetypes in Fig. \ref{fig:qm9selection}. In our case, we perform model selection by observing where the MAE converges (starting from 20 archetypes) to select the optimal number of archetypes. Obviously, if the number of archetypes is smaller, it becomes more difficult to reconstruct the data. This stems from the fact there exist a large number of molecules with almost the same heat capacity but with a different shape. Thus, molecules with different shapes are mapped to archetypes with the same heat capacity which makes it hard to resolve the many-to-one mapping in the latent space. 

In \textbf{Experiment 2}, we identify archetypal molecules that are associated with a particular heat capacity. In this setting, we focus on 20 archetypes (Fig. \ref{fig:qm9selection}) to obtain the optimal exploration-exploitation trade-off. While focusing only on a small selection of archetypes, we provide the full list in the supplement. In chemistry, the heat capacity is defined as $C_v = \dfrac{d\epsilon}{dT} \bigm|_{v=const}$ where $\epsilon$ denotes the energy of a molecule and $T$ is the temperature. The energy can be further decomposed into $\epsilon = \epsilon^{Tr}+\epsilon^R+\epsilon^V+\epsilon^E$ where $Tr$ depicts translation, $R$ rotation, $V$ vibration and $E$ the electric contribution, respectively \cite{atkins2010atkins,tinoco2002physical}. Building upon this knowledge, we compare different archetypal molecules associated with a particular heat capacity (Fig. \ref{fig:comparisions}). Here, the rows correspond to archetypes and the columns depict the three closest test molecules to the archetype. In Fig. \ref{figure:case1} we illustrate two archetypes with a high and low heat capacity. The first row archetype has a lower heat capacity because of its shorter chain and more double bonds. Due to these properties, the archetype is more stable which results in a lower vibrational energy $V$ and subsequently in a lower heat capacity. Fig. \ref{figure:case2} plots both a non-linear and a linear archetypal molecule with the same atomic mass. Here, the linear molecule loses one of its rotational modes due to its geometry. Therefore, the second row archetype has a lower rotational energy $R$ compared to the first row archetype, leading to a lower heat capacity. 

In \textbf{Experiment 3}, we focus on the interpolation between two archetypes. We do so by plotting the test samples which are closest to the linear connection between the two archetypes. Here, we observe a smooth transition from a ring molecule to a linear molecule with the same heat capacity. Along these archetypes, which both are similar in heat capacities but differ in shape, a molecule can only change its shape but it cannot go beyond a particular heat capacity. Results are shown in Fig. \ref{fig:interpolation}. 

Finally, in \textbf{Experiment 4}, we demonstrate that our model structures latent spaces according to the side information provided. Consequently, a molecule being a mxiture of archetypes with respect to heat capacity might become archetypal with respect to another property. Here, we compare the discovered archetypes for two specific chemical properties, heat capacity and band gap energy. In Fig. \ref{fig:side}, we plot the archetypes with the highest and lowest heat capacity (Fig. \ref{figure:heatcap}) and the highest and lowest band gap energy (Fig. \ref{figure:gap}), respectively. The extreme archetypes significantly differ in their structure as well as their atomic composition based on their property. For example, the archetype with low heat capacity are rather small with only a few C and O atoms. In contrast, the archetype with a low band gap energy are composed as rings with N and H atoms. A more detailed comparison between all archetypes can be found in the supplement. 

\begin{figure*}[!h]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/long_chain.pdf}
        \caption{}\label{figure:heatcap}
    \end{subfigure} \hspace{.35cm}
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/gap_ext.pdf}
        \caption{}\label{figure:gap}
    \end{subfigure}
    \caption{The panels illustrate a comparison between archetypes with side information with the highest and lowest property values. Here, the labels correspond to the heat capacity (a) and the band gap energy (b). The columns denote the molecules that are closest to a specific certain and the rows denote the archetypes. Panel (a) depicts archetypal heat capicity molecules and Panel (b) shows archetypal band gap energy molecules.}
    \label{fig:side}
\end{figure*}

%Last, we consider in Subfigure \ref{figure:case2} two archetypes with different weight. These molecules absorb the same energy due to their form.
%Figure \ref{fig:comparisions} illustrates comparisons between archetypal molecules and their heat capacity.

%This is in particular useful to uncover materials that heat up quickly (e.g. cooking pots) or slowly (e.g. coolants for cars or machines).

%Stability of archetypes is influenced by the discriminatory power of the provided side information. A given scalar-valued side information, e.g. the heat %capacity $C_v$, is associated with a certain degree of structural variability such that simultaneous prediction of $C_v$ and molecule reconstruction might %lead to variations in the obtained archetypes. To test the stability of archetypes, we have retrained DeepAA seven times and qualitatively observed that %archetypes associated with lowest and highest heat capacities are structurally very similar between independent runs (see appendix). This structural >%similarity also extends to other archetypes in between these extremes. However, there are a some archetypes emerging which cannot be related to archetypes of %other runs. From this we conclude that side information is capable of providing (task- or side-information-specific) archetypes which to some degree can be %considered stable.

==> 128-paper (2)/a04_deepAT_CONCLUSION_gcpr2019.tex <==
\section{Conclusion}
\label{sec_concl}
In this paper, we introduced a novel neural network based approach to learn a structured latent representation of a given dataset. The structure we impose onto the latent space allows to characterize this space through its most extremal or \textit{archetypal} representatives. In doing so, we build upon the linear AA approach and combine this concept with the deep IB principle to obtain a non-linear archetype model. In contrast to the classical approach our method offers three advantages: First, our model introduces a data-driven representation learning which reduces the dependence on expert knowledge. Second, we learn appropriate transformations to obtain meaningful archetypes even on non-linear data manifolds. Third, we are able to incorporate side information into the learning process. This counteracts overly flexible deep neural networks in order to identify meaningful archetypes with specific properties and facilitate an interpretable exploration of the latent space representations. Our experiment on the QM9 molecular dataset demonstrate the applicability of our method in an important real world setting. 

%explain the latent representation in terms of convex combinations of extremal points in latent space.    types, archetypes which is inspired by
%explain datapoints as convex combinations of archetypes which is inspired by studies of evolutionary trade-offs. In doing so, we build upon the linear AA %approach and combine this concept with the deep IB principle to obtain a non-linear archetype model. In contrast to the classical approach our method offers %three advantages: First, our model introduces a data-driven representation learning, which reduces expert knowledge. Second, we learn appropriate %transformations when combining features of different types. Third, we are able to incorporate side information into the learning process to identify archetypes %with specific properties. Our diverse experiments on biological, vision and chemical datasets demonstrate the applicability of our method in real world %settings. For future work, we would like to apply our deep archetype model to text data.

\paragraph{\textbf{Acknowledgements.}}
S.K. is partially supported by the the Swiss National Science Foundation project CR32I2 159682. M.S. is supported by the Swiss National Science Foundation grant 407540 167333 as part of the Swiss National Research Programme NRP 75 "Big Data". M.W. is partially supported by the NCCR MARVEL, funded by the Swiss National Science Foundation and SNSF grant 51MRP0158328 (SystemsX.ch).

==> a03_deepAT_EXPERIMENTS_Bats_gcpr2019.tex <==
\subsection{Representation Learning for \textit{Microchiroptera}}
\label{subsec_deepBats}
%
Based on expert knowledge \textit{body mass} and \textit{wing aspect ratio} were chosen to be the two most important features relating to the \textit{dominant food habit} of Microchiroptera, see Fig. \ref{fig:bats138}. But \cite{norberg1987} have collected six additional measurements on each species. These are \textit{wing span, wing area, wing loading, tip length ratio, tip area ratio and tip shape index}. Arguably, more meaningful archetypes may be found by learning an appropriate representation based on \textit{all} available measurements. We use \textit{DeepAA} to learn such a representation. Our encoder is shown in Fig. \ref{fig:at-supervised-arch}. Both encoder and decoder are parametrized by two feed-forward neural networks with two hidden layers each. We train the VAE for 200 epochs (learning rate: $1\text{e-}3$, batch size: 60) in a side information setting with the \textit{dominant food habit} as the additional information. 
%
%Based on physical intuition it is sensible to assume that bats whose primary food source are other flying %animals have evolved to be more aerodynamical than bats living off plant material.
%
\begin{figure}[h!]
\begin{center}
   \includegraphics[scale=.385]{bats138_deep}
\end{center}
\vspace{-1.8em}
\caption{\textit{DeepAA} finds a organisation of species not unsimilar to linear AA: Insectivores and frugivores populate opposite ends of the Pareto front. But the interesting insight is the representation associated with the latent space ordering found by \textit{DeepAA}. While linear AA was forced to find the best possible representation in the space of \textit{Wing Aspect Ratio} and \textit{Body Mass}, \textit{DeepAA} was free to learn a representation which included two additional features, i.e. $Wing Loading$ and $Tip Shape Index$. Based on these features \textit{DeepAA} was able to learn a richer representation which is in much agreement with the finding of \cite{norberg1987}, as discussed in the paragraph \textit{Results and Discussion}.}
\label{fig:bats138_deep}
\end{figure}
%
%
%\caption{Phenospace of 138 species of Microchiroptera. The dominant food habit of each %species, and thereby the ability to procure this food source, is linked to the morphology of %the animals, e.g. a higher \textit{Wing Aspect Ratio} corresponds with the greater aerodynamic %efficiency needed to chase high flying insects. Archetypes are extreme types, optimized to %perform a single task. Proximity of a species to an archetype quantifies the level of %adaptation this species has undergone with respect to the archetypal task.}
%
%
In order to compare to the results based on linear AA, we choose the same number of archetypes as in Fig. \ref{fig:bats138}. The representation learned by \textit{DeepAA} is shown in Fig. \ref{fig:bats138_deep}. By running the latent \textit{Archetypes A, B} and \textit{C} through the decoder of our trained VAE we obtain three sets of eight \textit{generated} features. Each set represents the traits of an archetypal species in terms of the eight measures introduced by \cite{norberg1987}. For these three species we analyze by how much each feature changes. This allows us to deduce the most important measures characterizing the relation between \textit{food habit} and \textit{morphology}.
%
\begin{table}%[b!]
\caption{Characteristic traits of the archetypes identified in Fig. \ref{fig:bats138_deep} and the task each archetypal species is optimized to perform.}
\label{tbl_deep_traits}
\vskip 0.05in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Measure & importance & A & B & C \\
\midrule
total mass        & 35\% & med  & low & high \\
wing area         & 30\% & low  & med & high \\
wing loading      & 15\% & low  & med & high \\
wing span         & 10\% & low  & low & high \\
tip shape index   & 10\% & high & med & low \\
%tip length ratio  & -- & & & \\
%tip area ratio    & -- & & & \\
%ing aspect ratio & -- & & & \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%
\paragraph{Results and Discussion} Our results are shown in Table \ref{tbl_deep_traits}. For each measure we consider the largest relative change with respect to the archetypes and take the magnitude of these changes as a proxy for feature importance. Similar to Fig. \ref{fig:bats138}, we find that \textit{total mass} is the most important feature: The heavier a bat the more likely it is to be a frugivore -- a result consistent with linear AA. But in contrast to the linear case \textit{DeepAA} does not consider \textit{wing aspect ratio}. Instead \textit{wing area} and \textit{wing span} are deemed important. But as \textit{wing aspect ratio} is simply the square of the \textit{wing span} divided by the \textit{wing area}, one could argue that \textit{DeepAA} captures the influence of \textit{wing aspect ratio} nonetheless. 
A novel insight produced by \textit{DeepAA} is the importance of two additional features, namely \textit{wing loading} and \textit{tip shape index}. According to \cite{norberg1987}, as wing loading increases, the bat must fly faster and expend more energy, and the range of accessible flight behavior is reduced. As \textit{Archetype A} has low \textit{wing loading}, thereby enabling various flight behaviors, it makes sense that this archetype can accommodate the largest variation in food habits, i.e. frugivore, nectarivore, insectivore, pescivore, carnivore and sanguivore are all found in proximity to \textit{Archetype A}. Regarding \textit{tip shape index}, \cite{norberg1987} find that it is inversely correlated with flight speed. They further state that flight speed increases significantly with \textit{wing loading}. As shown in Table \ref{tbl_deep_traits}, this is exactly the inverse relation learned by \textit{DeepAA} -- high \textit{wing loading} and low \textit{tip shape index} for \textit{Archetype A} while the inverse is true for \textit{Archetype C}. The learned representation is thus in very good agreement with the various trade-offs found by \cite{norberg1987}. But \textit{DeepAA} did not only find a richer and arguably more meaningful representation than linear AA, it also learned the appropriate scaling when combining the different features. By contrast, in linear AA one had to know \textit{beforehand} that \textit{total mass} would need to enter the model logarithmically.


%Consitent with the observation/calc from norberg, tip is....

%, low flight speed is correlated with large wingtip shape index, I

%speed increased significantly with wing loading

%Mass-carrying ability will be linked most closely with wing loading. As wing loading
%increases, the bat must fly faster and expend more energy, and the range of accessible flight
%ehaviour is reduced until flight is no longer possible. Because they habitually fly with
%ubstantial loads, we expect carnivores to have relatively low wing loading. Large wingspan
